Predicting Domain Generation Algorithms with Long Short-Term Memory Networks

Various families of malware use domain generation algorithms (DGAs) to generate a large number of pseudo-random domain names to connect to a command and control (C&C) server. In order to block DGA C&C traffic, security organizations must first discover the algorithm by reverse engineering malware samples, then generating a list of domains for a given seed. The domains are then either preregistered or published in a DNS blacklist. This process is not only tedious, but can be readily circumvented by malware authors using a large number of seeds in algorithms with multivariate recurrence properties (e.g., banjori) or by using a dynamic list of seeds (e.g., bedep). Another technique to stop malware from using DGAs is to intercept DNS queries on a network and predict whether domains are DGA generated. Such a technique will alert network administrators to the presence of malware on their networks. In addition, if the predictor can also accurately predict the family of DGAs, then network administrators can also be alerted to the type of malware that is on their networks. This paper presents a DGA classifier that leverages long short-term memory (LSTM) networks to predict DGAs and their respective families without the need for a priori feature extraction. Results are significantly better than state-of-the-art techniques, providing 0.9993 area under the receiver operating characteristic curve for binary classification and a micro-averaged F1 score of 0.9906. In other terms, the LSTM technique can provide a 90% detection rate with a 1:10000 false positive (FP) rate---a twenty times FP improvement over comparable methods. Experiments in this paper are run on open datasets and code snippets are provided to reproduce the results.

==> CNS16/abstract.tex <==
Various families of malware use domain generation algorithms (DGAs) to periodically generate a large number of domain names to connect to a command and control server.  One technique to defeat such malware is to pre-register all domain names that it generates.  However, malware using DGAs have the potential to generate tens of thousands of domains per day making it near impossible to proactively register malicious domains. In addition, DGAs can be modified such that defenders can no longer predict which DGAs will be produced on a given day.  Another technique to stop malware from using DGAs is to intercept DNS traffic on a network and predict whether domains are DGAs.  Such a technique will alert network administrators to the presence of malware on their networks.  In addition, if this predictor can also accurately predict the family of DGAs, then network administrators can also be alerted to the type of malware that is on their networks.  This paper presents a DGA prediction technique that uses long short-term memory (LSTM) networks to predict DGAs and their respective families.  Results are significantly better than state-of-the-art techniques with an improvement of XX\% as measured by the area under the curve of the receiver operating characteristic.  Experiments in this paper are run on open datasets and code snippets are provided to reproduce the results.

==> CNS16/conclusion.tex <==
our conclusions

==> CNS16/expsetup.tex <==
The proposed technique is evaluating using three different experimental designs:

\begin{enumerate}
  \item Binary classification,
  \item binary, leave-one-out classification, and
  \item multi-class classification. 
\end{enumerate}

The binary classification experimental design tests each DGA classifier for it's ability to make an accurate binary decision: DGA or not DGA.  The DGA class consists of domains from all families in our training set.  This experiment is run using n-fold cross validation with ten folds.

The binary, leave-one-out classification experimental design tests each classifiers' robustness to new DGA families.  For each DGA family, all samples from that family are removed from the training set.  The remaining families are only included in the training set (i.e., not evaluated in the test set).  The removed family of DGAs is then evaluated along with a hold out set of domains that are not DGAs.  Each experiment per family is run using n-fold cross validation with ten folds.

The multi-class classification design tests each DGA classifier for it's ability to make an accurate decision on the family of DGA.  Domains that are not DGAs are removed from this design (i.e., we only train and test on DGAs for the multi-class classifier).  The HMM and random forest DGA classifiers use One vs. Rest while the LSTM classifier does a direct multi-class classification.  This experiment is run using n-fold cross validation with ten folds.

\subsection{Data}
The experimental designs use data from two sources.

\begin{enumerate}
  \item The Alexa top 1 million domains \cite{Alexa1M} are used for training domains that are not DGAs.
  \item The OSINT DGA feed from Bambenek Consulting \cite{dgafeed} is used for DGA domains.
\end{enumerate}

The OSINT DGA feed consists of 30 families of DGAs with a varying number of examples from each class.  This feed contains approximately 750,000 DGA examples.

 

==> CNS16/introduction.tex <==
Domain generation algorithms (DGAs) are used by many malware families to make preemptive defenses difficult.  Domains are generated pseudo-randomly in bulk (hundreds to tens-of-thousands per day) by a piece of malware.  This piece of malware then attempts to connect to all or a portion of these generated domains in hopes of finding a command and control server from which it can update, upload gathered intelligence, or pursue other malicious activities.  The malicious actor only needs to register a small number of these domains to be successful.  However, all the domains must be sinkholed, registered, or blacklisted before they go into use in order to preemptively defeat such an attack.  This defense becomes increasingly difficult with an increasing number of generated domains per day. 

Authors in \cite{kuhrer2014paint} presented a thorough review of the efficacy of blacklists.  As a part of this review, authors analyzed both public and private blacklists for DGA coverage, i.e., how many domains generated by DGAs were contained in blacklists.  Public blacklists were surprisingly lacking in terms of DGA coverage with less than 1.2\% of DGAs analyzed by the authors being contained in any of the blacklists.  Vendor provided blacklists fared better, but had mixed results over familes with coverage varying from 0\% to 99.5\%.  These results suggest that blacklists are useful, but must be supplemented by other techniques to provide a more adequate level of protection.

Another approach to combating malware using DGAs is to build a DGA classifier.  This classifier can live in the network sniffing out DNS requests and looking for DGAs.  When DGAs are detected, the classifier notifies other automated tools or network administrators to further investigate the origin of a DGA.  This paper presents such a technique using Long Short-Term Memory networks (LSTMs) to classify DGAs.  This technique has three significant advantages over other techniques in the literature.  First, LSTMs work on raw featureless data.  The presented technique trains on raw domain names (e.g., endgame.com, google.com, facebook.com, etc.).  If a new family of DGA appears, then the classifier can be retrained without the tedious step of hand picking features.  Second, the presented technique works significantly better than hand tuned parameters.  Third, the technique also works on multi-class classification.  Therefore, the algorithm can not only give a binary decision of whether a domain is DGA or not, but it can accurately predict a DGA's origin.

Previous approaches to classifying DGAs typically use hand picked features (such as entropy, length, and vowel to consonant ratio) that are fed into a general classifier, such as random trees.  This approach generally produces good classification results, however, a large amount of manual work is required to extract the right features. In addition, adversaries can produce new DGAs that are undetectable from a known set of features; cat and mouse.  LSTMs, on the other hand, need no manual feature selection and a classifier can be simply rebuilt in the presence of new DGA families.

Other approaches make classifications in large sets of domains \cite{antonakakis2012throw, yadav2012detecting, nelms2013execscent}.  These sets are broken down into groupings using clustering with the intent to generate statistical properties of each grouping.  Classification is accomplished by generating templates during training and using statistical tests (such as Kullback-Leibler divergence) to classify groups of potential DGAs.  In addition, these techniques take in contextual information such as HTTP headers to further improve performance. The LSTM DGA classifier presented in this paper works on individual samples of domains and takes in no contextual information; just the domain name.  The LSTM method presented in this paper is not meant to replace the aforementioned techniques, but used symbiotically as suggested in \cite{antonakakis2012throw}.  I.e., this technique can be used in conjunction with the aforementioned techniques to further improve the efficacy of locating DGAs.

This paper makes three main contributions:

\begin{enumerate}
  \item Presents an LSTM Network to predict DGA generated domains
  \item Presents complete experimental results showing significant improvements over previous techniques in the literature using open datasets
  \item Provides source code to reproduce results
\end{enumerate}

Source code is provided in Python and built on the open source Keras framework \cite{chollet2016} allowing for easy reproducibility.  Experiments were run on GPU hardware for performance reasons, but its possible to run all experiments on commodity dektop or laptop hardware.  Details of reproducing the results, as well as suggestions for running without GPUs is given in sections \ref{method} and \ref{expsetup}.  An overview of LSTMs, the Keras framework and previous work is discussed in section \ref{background}. Full results are given in section \ref{results} with suggestions for future work given in section \ref{conclusion}.


==> CNS16/method.tex <==
We employ an LSTM network for detecting DGAs.  The model has the following advantages:
\begin{itemize}
\item the model accepts variable-length character sequences as input, so that there is no auxiliary requirement for feature extraction\footnote{In experiments, we employ a trivial pre-processing step to remove top-level domains.};
\item the model is very compact, comprised simply of an input layer of LSTMs followed by a fully connected output layer that is simple logistic (or for multi-class, multinomial logistic) regression; and
\item although training on a large dataset is computationally intensive, the shallow structure allows for very fast query times.
\end{itemize}
To prevent overfitting when training neural networks, it is common practice to employ dropout. Dropout consists of randomly removing edges between layers in a network.  We apply dropout after the layer of LSTMs prior to logistic regression.

\begin{figure}
\centering
\includegraphics[scale=0.5]{figs/model}
\caption{Our model consists of (top layer) an LSTM layer that serves essentially as a feature extractor for (bottom layer) a logistic regression classifier.}
\end{figure}

The LSTM layer can be thought of as implicit feature extraction as opposed to explicit feature extraction (e.g., \textit{n}-grams) used in other approaches.  Rather than represent domain names explicitly as a bag of bigrams, for example, the LSTM learns patterns of characters that maximize the performance of the second classification layer.  \textbf{To do:} We show a comparison of LSTM features--with instances where the neurons have high activity--to a bigram model with logistic regression.

==> CNS16/relatedwork.tex <==
In a variety of natural language tasks, recurrent neural networks (RNNs) have been used to capture temporal relationships between tokens in a sequence \cite{robinson1994application,mikolov2010recurrent,graves2012sequence,bengio2013advances}.  When training a traditional RNN, the gradient magnitude may tend towards zero, leading to the well-known problem of \textit{vanishing gradients}.  This makes learning long-term dependencies in an RNN difficult to achieve.  

The problem of vanishing gradients is a key motivation behind the design of the Long Short-Term Memory (LSTM) cell \cite{hochreiter1997long, gers2000learning, gers2003learning}, which consists of an input gate, a neuron with a self-recurrent connection, a forget gate and an output gate.  The input gate modulates to what extend the cell's state is modified by an input.  The self-recurrent gate retains state between adjacent timesteps.  The output gate modulates to what extent the cell's state is passed along to other neurons.  The forget gate modulates the memory cell's self-recurrent connection, providing a mechanism whereby the cell's state can be reset.

%\textbf{To do:} I have adequate citations, but will flesh out the descriptions.  One of the better descriptions of LSTMs is actually at \url{http://deeplearning.net/tutorial/lstm.html}

==> CNS16/results.tex <==
Our results
